Verification of Neural Networks against Convolutional Perturbations via Parameterised Kernels

We develop a method for the efficient verification of neural networks against convolutional perturbations such as blurring or sharpening. To define input perturbations we use well-known camera shake, box blur and sharpen kernels. We demonstrate that these kernels can be linearly parameterised in a way that allows for a variation of the perturbation strength while preserving desired kernel properties. To facilitate their use in neural network verification, we develop an efficient way of convolving a given input with these parameterised kernels. The result of this convolution can be used to encode the perturbation in a verification setting by prepending a linear layer to a given network. This leads to tight bounds and a high effectiveness in the resulting verification step. We add further precision by employing input splitting as a branch and bound strategy. We demonstrate that we are able to verify robustness on a number of standard benchmarks where the baseline is unable to provide any safety certificates. To the best of our knowledge, this is the first solution for verifying robustness against specific convolutional perturbations such as camera shake.

==> figures/convolution.tex <==
\begin{figure*}[!htb]
\centering
\begin{adjustbox}{width=.6\textwidth, center}
\begin{tikzpicture}

% Define colours to use
\def\imcolour{NavyBlue}
\def\kernelcolour{Orange}
\def\resultcolour{OliveGreen}
\def\minsize{9mm}

\matrix (mtr) [matrix of nodes,row sep=-\pgflinewidth, nodes={draw, minimum size=\minsize, anchor=center}]
{
|[fill=\imcolour!30]| $5$ & |[fill=\imcolour!30]| $2$ & |[fill=\imcolour!30]| $2$ & $8$\\
|[fill=\imcolour!30]| $2$ & |[fill=\imcolour!30]| $0$ & |[fill=\imcolour!30]| $0$ & $9$\\
|[fill=\imcolour!30]| $3$ & |[fill=\imcolour!30]| $7$ & |[fill=\imcolour!30]| $1$ & $3$\\
$3$ & $2$ & $5$ & $7$\\
};

\draw[very thick, \imcolour] (mtr-1-1.north west) rectangle (mtr-3-3.south east);

\node [below= 2em of mtr-4-3.south west] (lm) {$\bf I$};

\node[right = 0.2em of mtr] (str) {$*$};

\matrix (K) [right=0.2em of str,matrix of nodes,row sep=-\pgflinewidth, nodes={draw, fill=\kernelcolour!30, minimum size=\minsize, anchor=center}]
{
$0$ & $\frac{1}{3}$ & $0$ \\
$0$ & $\frac{1}{3}$ & $0$ \\
$0$ & $\frac{1}{3}$ & $0$\\
};
\node [below = 3.28em of K-3-2.south] (lk) {$\bf K$};

\node [right = 0.2em of K] (eq) {$=$};

\matrix (ret) [right=0.2em of eq,matrix of nodes,row sep=-\pgflinewidth, nodes={draw, minimum size=\minsize, anchor=center}]
{
|[fill=\resultcolour!30]| $3$ & $1$ \\
$3$ & $2$\\
};
\node [below = 4.56em of ret-2-2.south west] (lim) {${\bf I} * {\bf K}$};

\draw[very thick, \resultcolour] (ret-1-1.north west) rectangle (ret-1-1.south east);

\draw[dashed, \kernelcolour, thick] (mtr-1-1.north west) -- (K-1-1.north west);
\draw[dashed, \kernelcolour, thick] (mtr-3-1.south west) -- (K-3-1.south west);
\draw[dashed, \kernelcolour, thick] (mtr-1-3.north east) -- (K-1-3.north east);
\draw[dashed, \kernelcolour, thick] (mtr-3-3.south east) -- (K-3-3.south east);

\draw[dashed, \resultcolour, thick] (ret-1-1.north west) -- (K-1-1.north west);
\draw[dashed, \resultcolour, thick] (ret-1-1.south west) -- (K-3-1.south west);
\draw[dashed, \resultcolour, thick] (ret-1-1.north east) -- (K-1-3.north east);
\draw[dashed, \resultcolour, thick] (ret-1-1.south east) -- (K-3-3.south east);

\matrix (K) [right=0.2em of str,matrix of nodes,row sep=-\pgflinewidth, nodes={draw, fill=\kernelcolour!10, minimum size=\minsize, anchor=center}]
{
$0$ & $\frac{1}{3}$ & $0$ \\
$0$ & $\frac{1}{3}$ & $0$ \\
$0$ & $\frac{1}{3}$ & $0$ \\
};

\draw[very thick, \kernelcolour] (K-1-1.north west) rectangle (K-3-3.south east);

%\node[anchor=south east, inner sep=0.01em, \kernelcolour] at (mtr-1-1.south east) (xx) {\scalebox{.5}{$\times 1$}};
%\node[anchor=south east, inner sep=0.01em, \kernelcolour] at (mtr-1-2.south east) (xx) {\scalebox{.5}{$\times 0$}};
%\node[anchor=south east, inner sep=0.01em, \kernelcolour] at (mtr-1-3.south east) (xx) {\scalebox{.5}{$\times 1$}};
%\node[anchor=south east, inner sep=0.01em, \kernelcolour] at (mtr-2-1.south east) (xx) {\scalebox{.5}{$\times 0$}};
%\node[anchor=south east, inner sep=0.01em, \kernelcolour] at (mtr-2-2.south east) (xx) {\scalebox{.5}{$\times 1$}};
%\node[anchor=south east, inner sep=0.01em, \kernelcolour] at (mtr-2-3.south east) (xx) {\scalebox{.5}{$\times 0$}};
%\node[anchor=south east, inner sep=0.01em, \kernelcolour] at (mtr-3-1.south east) (xx) {\scalebox{.5}{$\times 1$}};
%\node[anchor=south east, inner sep=0.01em, \kernelcolour] at (mtr-3-2.south east) (xx) {\scalebox{.5}{$\times 0$}};
%\node[anchor=south east, inner sep=0.01em, \kernelcolour] at (mtr-3-3.south east) (xx) {\scalebox{.5}{$\times 0$}};

\end{tikzpicture}
\end{adjustbox}
\caption{Convolution}
\label{fig:convolution}
\end{figure*}

